An Approach for Generating Families of Energetically Optimal Gaits from Passive Dynamic Walking Gaits

For a class of biped robots with impulsive dynamics and a non-empty set of passive gaits (unactuated, periodic motions of the biped model), we present a method for computing continuous families of locally optimal gaits with respect to a class of commonly used energetic cost functions (e.g., the integral of torque-squared). We compute these families using only the passive gaits of the biped, which are globally optimal gaits with respect to these cost functions. Our approach fills in an important gap in the literature when computing a library of locally optimal gaits, which often do not make use of these globally optimal solutions as seed values. We demonstrate our approach on a well-studied two-link biped model.

==> epsilon.tex <==

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{The Space of Parameterized Trajectories}
% \begin{mydef}
% Let $x_0 \in \X$ be a pre-impact state, $\tau \in \R$
% be a switching time, and $\mu \in \R^k$ be a vector of input
% parameters.  A biped's \emph{state-time-control space} $\Space$ is a finite parameter vector space $\Space \subseteq \X \times \R \times \R^k$.
% \end{mydef}

% A point $c \in \Space$, where $c = \xtu$, defines the evolution of a hybrid
% trajectory $x(t) \in \X$ starting from $x_0$ at time $t = t_0$ with switching
% times in $\tau$, and input parameters $\mu$.

% \begin{mydef}
% \label{def:P}
% A point $c = \xtu \in \Space$ is a \emph{gait} of the biped if it is a root of the \emph{periodicity map} $P: \Space \rightarrow \Rx$ such that $P(c) = \flow[2 \tau] - x_0 = 0$.  The \emph{set of all gaits} $\G$ and the \emph{set of passive dynamic walking gaits} $\Gpass$ are then 
% \begin{align}
%     \G &= \pre{P} = \{c \in \Space: P(c) = 0\}, \\
%     \Gpass &= \{c \in \G: u(t) = 0, t \in \R \}.
% \end{align}
% \end{mydef}

% \begin{mydef} \cite{Spivak1965}
% For $c \in \G$, if $\rank(\pd{P}{c}(c)) = k + 1$, then 
% \begin{enumerate}
%     \item $c$ is a \emph{regular point} of $\G$ (and a \emph{singular point} otherwise),
%     \item the tangent space of $\G$ at $c$, $T_c\G$, is equal to the null space of $\pd{P}{c}$ (i.e., $T_c\G = \Null(\pd{P}{c})$), and
%     \item there exists a neighborhood of regular points containing $c$ that form a differentiable manifold in $\G$.
% \end{enumerate}
% \end{mydef}

% Given that the flow and hence $P$ is differentiable (Assumption~\ref{as:diff}), the gaits in $\G$ form connected components of gaits.  In general, a connected component of $\G$ consist of $(k+1)$-dimensional differentiable manifolds of gaits glued together at singular points of the periodicity map $P$.  These manifolds are the \textit{branches} of the connected component.

% Ultimately, we aim to trace optimal gaits in user-defined slices of a connected component of $\G$.  We identify user-defined slices with the map $M$
% \begin{equation}
% \label{eq:M}
% M(c) = [P^T(c), \Phi^T(c)]^T \in \Rlam,
% \end{equation}
% where $\Phi(c) \in \R^{(\n{\lambda} - 2n)}$ ($\n{\lambda} - 2n > 0$) is a set of user-defined constraints.  For example, to trace gaits that walk on a fixed slope $\sigma_0 \in \R$ and average walking speed $v_0 \in \R$, we have 
% \begin{equation}
%     \label{eq:Phi}
%     \Phi(c) = [\sigma(c) - \sigma_0, v_\text{avg}(c) - v_0]^T,
% \end{equation}
% where ${\fun{\sigma}{\G}{\R}}$ and ${\fun{v_\text{avg}}{\G}{\R}}$ are a gait's slope and average walking speed, respectively (see Appendix).

% %Given $M$, the next step is to identify optimal gaits in $\pre{M} \subset \G$ for a given cost function $J(c) \in \R$.

% \subsection{Optimal Trajectories in the Gait Space}
% When it comes to generating optimal gaits in $\G$, the map $M$ of Equation~\eqref{eq:M} can be treated as the (equality) constraints to an optimization problem $OP$ such that
% \begin{customopti}
%         {optimize}{c \in \Space}{J(c),}{\label{opti:op}}{OP:}
%         \addConstraint{M(c)}{= 0,}
% \end{customopti}
% where $c$ is a vector of decision variables, $J(c) \in \R$ is a given cost function, and $M$ is a vector of equality constraints.

% \begin{myrem}
% \label{rem:stationary}
% Our formulation of $OP$ only identifies stationary points.  We do not distinguish between optimal points that are minima, maxima, or neither.
% \end{myrem}

% \begin{mydef}
% Given the optimization problem $OP$ of Equation~\eqref{opti:op}, a trajectory $c \in \Space$ is an \emph{optimal gait} in $\pre{M} \subset \G$ if $c$ satisfies the first-order optimality conditions (FOC) \cite{Nocedal1999}
% \begin{equation}
% \label{eq:oc}
%     M(c) = 0, \quad \oc = 0,
% \end{equation}
% where $\lambda \in \Rlam$ is a vector of Lagrange multipliers.
% \end{mydef}
% This leads to the set of optimal gaits in a subspace of $\G \times \Rn{\lambda}$ that are the roots of the map $\dJ$, where
% \begin{equation}
% \label{eq:dJ}
% \dJ = \left[ M^T(c), \left( \oc \right)^T \right]^T.
% \end{equation}
% In other words, the map $\dJ$ consists of the FOC for $OP$.  Thus, Equation~\eqref{eq:dJ} transforms an optimization problem into a map $\dJ$ with the same solution set in $\Space$.

% \begin{myprop}
% [Can we state a non-obvious proposition that gaurantees that PDW are optimal w.r.t. J]?  All gaits in the set of PDW gaits $\Gpass$ are optimal with respect to cost function $J(c) = J(u(t; c))$, if $\text{infinum}(J) = 0$ and $J(u = 0) = 0$.
% \end{myprop}

% \begin{myprop}
% \label{prop:iso}
% Let $(c, \lambda) \in \predJ$ be an optimal pair of the cost function $J(c) \in \R$ subject to constraints $M(c) = 0$.  If the pair $(c, \lambda)$ is a regular point of $\dJ$, then it is also an isolated point in $\predJ$.
% \end{myprop}
% \begin{proof}
% The tangent space $T_{(c, \lambda)}\dJ$ represents all of the feasible directions we can move in without violating the FOC (Equation~\ref{eq:oc}).  At a regular point, the tangent space equals the null space.  The null space is empty because the Jacobian of $\dJ$ is square and has maximal rank, hence $(c, \lambda)$ is an isolated point in $\predJ$.
% \end{proof}
% Stated differently, the regular points of $\predJ$ do not form a continuous family of gaits.  Instead of trying to find gaits in an isolated set, we instead embed the $OP$ into a 1D family of optimization problems in such a way that we can connect gaits in $\predJ$ to gaits in $\Gpass$.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Problem Statement}
% \label{ssec:prob}
% Given:
% \begin{itemize}
% 	\item a hybrid model $\Sigma$ of an $n$-degree-of-freedom biped with $m$ switching times, and $k$ control and design parameters,
% 	\item a set of $p$ basis functions $\B_1$, $\ldots$, $\B_p$ for defining the input $u(t) \in \Rq$,  
% 	\item a space $\Space \subset \Rc$ of parameterized trajectories with nonempty sets of gaits $\G$ and $\Gpass$, and
% 	\item twice-differentiable cost function $\fun{J}{\Space}{\R}$ and user-defined map $\fun{\Phi}{\Space}{\R^{\nlam - 2n}}$ ($\nlam - 2n > 0$) for defining $M$ of Equation~\eqref{eq:M}.
% \end{itemize}
% Find: A continuous path $\fun{p}{[0, 1]}{\G}$ such that
% \begin{itemize}
%     \item $p(0) \in \predJ$, 
%     \item $p(1) \in \Gpass$, and
%     \item for all $\epsilon \in [0, 1]$, the gaits $p(\epsilon)$ are stationary points of the parametric optimization problem
% \begin{customopti}
%         {optimize}{(c, \lambda) \in \Space \times \Rlam}{J(c) + \lambda^T \Me(c),}{\label{opti:ope}}{\OPe:}
% \end{customopti}
% where $c$ is a vector of decision variables, $\epsilon \in \R$ is an indexing parameter such that $\Me(c) = [P^T(c), \Ie^T(c)]^T \in \Rlam$ is an indexed set of constraints with $\Ie$ defined in terms of $\epsilon$ and $\Phi$, $J(c) \in \R$ is the cost function, and $\lambda \in \Rlam$ is a vector of Lagrange multipliers.
% \end{itemize}

% In other words, the continuous parameter $\epsilon$ defines a family of optimization problems $OP(\epsilon)$ whose solution set are all gaits in $\G$.  The goal is to start with a PDW gait in $\Gpass$ and attempt to trace a path of optimal gaits that goes through a gait in $\predJ$ (see Figure~\ref{} for an illustration).  We outline such a process using numerical continuation methods in Section~\ref{sec:opt}, including a definition for the function $\Ie$.

% \begin{myrem}
% Given that we only trace stationary points (see Remark~\ref{rem:stationary}), identifying minima of $\OPe$ in $\Gm$, for example, would be a post-processing step in our framework.
% \end{myrem}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Generating A Set of Optimal Gaits}
% \label{sec:opt}
% We now describe how to embed the $OP$ into a 1D parameterized family of optimization problems $\OPe$ suitable for tracing curves of optimal gaits in $\G$.  The primary contribution of this section is the definition of a map $\Me$ that can trace a path of optimal gaits from PDW gaits to a gait in $\predJ$.  The algorithms in this section are from \cite{Rosa2021}, which we reuse to keep this paper self contained.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Specifying a 1D Family of Optimization Problems}
We embed the $OP$ into a 1D family of optimization families through the global homotopy map $\Me$
\begin{equation}
    \label{eq:Me}
    \Me(c, \lambda) = \dJ - \epsilon \dJ[M][(c_0, \lambda_0)],
\end{equation}
where $\epsilon \in \R$ is a real-valued index, $(c_0, \lambda_0) \in \Gpass \times \Rlam$ are the initial seed values, and $\dJ$ is defined in Equation~\eqref{eq:dJ}.

\begin{mydef}
For user-defined constraints $\Phi$, point $c_0 \in \Space$ and index $\epsilon \in \R$, let $\Ie(c)$ be an indexed set of constraints, where, up to a relabeling of the entries,
$$\Ie(c) = \Phi(c) - \epsilon \Phi(c_0) = [\Iz^T(c), \Inz^T(c) - \epsilon \Inz^T(c_0)]^T$$
such that $\Iz(c_0) = 0$ and $\Inz(c_0) \neq 0$.
\end{mydef}

\begin{myprop}
\label{prop:Me}
Given the map $\Me$, which is defined in terms of cost function $J$; periodicity map $P$; and user-defined constraints $\Phi$, if the seed value $(c_0, \lambda_0) \in \Space \times \Rlam$ satisfies
\begin{equation*}
    c_0 \in \Gpass, \oc[c_0][\lambda_0] = 0, \text{ and } M(c_0) \neq 0;
\end{equation*}
then curves traced using $\Me$ have the following homotopy properties:
\begin{enumerate}[label=HP\theenumi]
    \item \label{hp:0} at $\epsilon = 0$, we have an optimal solution to the underlying $OP$ of Equation~\ref{eq:oc},
    \item \label{hp:1} at $\epsilon = 1$, we start with a known optimal gait that is not a root of $\Phi$ (i.e., $\Inz(c_0) \neq 0$), but is optimal with respect to the set of constraints of $M_{\epsilon = 1}(c_0)$,
    \item  \label{hp:fam} the map solves a series of optimizations with an indexed family of constraints $\Inz(c) - \epsilon \Inz(c_0)$, and
    \item \label{hp:inv} every point on a curve defined implictly by $\Me$ satisfies $P(c) = 0$, $\Iz(c) = 0$, and $\oc = 0$.
\end{enumerate}
\end{myprop}

\begin{proof}
Homotopy Property \ref{hp:0} and \ref{hp:1} can be verified directly after plugging in the assumptions regarding the point $c_0$, in which case $\Me$ reduces to
\begin{equation}
\label{eq:simpleMe}
    \Me(c, \lambda) = \begin{bmatrix}
    P(c) \\
    \Iz(c) \\
    \Inz(c) - \epsilon \Inz(c_0) \\
    \oc
    \end{bmatrix}.
\end{equation}
After this simplification, we also see that Homotopy Property \ref{hp:fam} defines the set of constraints that vary throughout the continuation.  An example interpretation of this property is if $\Inz$ is a walking surface constraint $\Inz(c) = \sigma(c)$, then we would trace a set of gaits with a range of slopes $\sigma(c) \in [0, \sigma_0]$ for $\epsilon \in [0, 1]$.  Finally, Homotopy Property \ref{hp:inv} implies that the set of gaits we generate have a shared set of properties as the numerical continuation traces the resulting 1D curve starting from $(c_0, \lambda_0)$.  Most importantly, every gait is optimal with respect to cost $J(c)$ subject to constraints $M(c) - \epsilon M(c_0)$.
\end{proof}

In general, the utility of a global homotopy map is that we can choose any $c_0 \in \Space$ as a seed value for $\Me$ in an attempt to find a curve that goes through $c \in \predJ$, but in choosing our seed value $c \in \Gpass$, we establish several useful properties with respect to the potential curve traced using the map $\Me$.

\begin{myrem}
We have now introduced a set of variables $c$, $\lambda$, $\epsilon$, $c_0$, and $\lambda_0$ that are sometimes fixed and other times free.  In summary, for the purposes of numerical continuation, the variables $c$, $\lambda$, and $\epsilon$ are free variables to be determined by the numerical continuation algorithm.  However, when it comes to defining the stationary points of $OP$ and $\OPe$, $c$ and $\lambda$ are the decision variables and $\epsilon$ is a fixed parameter.  The values for $c_0$, and $\lambda_0$ are fixed in both cases.
\end{myrem}
